EventKG - the Hub of Event Knowledge on the Web - and Biographical Timeline Generation

One of the key requirements to facilitate the semantic analytics of information regarding contemporary and historical events on the Web, in the news and in social media is the availability of reference knowledge repositories containing comprehensive representations of events, entities and temporal relations. Existing knowledge graphs, with popular examples including DBpedia, YAGO and Wikidata, focus mostly on entity-centric information and are insufficient in terms of their coverage and completeness with respect to events and temporal relations. In this article we address this limitation, formalise the concept of a temporal knowledge graph and present its instantiation - EventKG. EventKG is a multilingual event-centric temporal knowledge graph that incorporates over 690 thousand events and over 2.3 million temporal relations obtained from several large-scale knowledge graphs and semi-structured sources and makes them available through a canonical RDF representation. Whereas popular entities often possess hundreds of relations within a temporal knowledge graph such as EventKG, generating a concise overview of the most important temporal relations for a given entity is a challenging task. In this article we demonstrate an application of EventKG to biographical timeline generation, where we adopt a distant supervision method to identify relations most relevant for an entity biography. Our evaluation results provide insights on the characteristics of EventKG and demonstrate the effectiveness of the proposed biographical timeline generation method.

==> 04e_limitations.tex <==
\section{Discussion}
\label{sec:discussion}

\revA{
\subsection{Discussion of Modelling Decisions}
\label{sec:discussion-modelling}

Driven by the objective to enable simple and efficient access to EventKG, we took decisions with respect to the modelling of time and relation information in the EventKG schema.

\subsubsection{Modelling Time Information}
\label{sec:discussion-modelling-time}
Event times can be modelled in different manners, e.g. to denote uncertainty. 
In the temporal slot filling task \cite{Surdeanu:2013}, time intervals are typically represented as quadruples (earliest and latest possible start/end time). 
In other work, the validity time of relations or events is modelled by a temporal distribution \cite{Li:2005}. 
Although there are possibilities to express dates with uncertainty (e.g. using the Extended Date Time Format \cite{EDTF}), our goal is to provide a precise knowledge graph that can be queried using standard means (such as temporal SPARQL queries) and therefore express each time interval with precise start and end dates. 
In the future work, information regarding the certainty or granularity of dates can be added to EventKG.

\subsubsection{Modelling Relations} 
\label{sec:discussion-modelling-relations}

Another modelling decision is the use of nodes in the knowledge graph to represent relations. %instead of expressing each temporal information as an event. 
For example, the start and end date of a ``spouse'' relation could refer to an event each (marriage and divorce) that could be modelled using even more detailed notions of the Simple Event Model. However, temporal relations inherently contain this information and can be used in a broader sense: In our use case of biographical timeline generation, the whole time span of two person's connection seems to be of a higher relevance in a person's biography than just the two events of marriage and divorce.
}


\subsection{Pipeline Discussion}
\label{sec:discussion-pipeline}

\ed{
\subsubsection{Integration of entities, events and relations}
\label{sec:discussion-integration-entities}

As described in Section \ref{sec:extraction}, integration of entities and events obtained from knowledge graphs is conducted using existing \textit{owl:sameAs} links. 
%
Currently, we do not consider any entity or event resolution techniques to integrate representations that refer to equivalent real-world objects and happenings for which such \textit{owl:sameAs} links are not provided. 
In the future work, entity resolution methods can be adopted 
to further increase the degree of integration in the EventKG. 
\todo[inline]{link to a method to resolve entities across KGs is needed here. }
}

\subsubsection{Integration of relations}
\label{sec:discussion-integration-relations}

As described in Section \ref{sec:extraction}, integration of relations is 
performed using a manually defined mapping table. 

==> timeline_size_distribution_wiki.tex <==
\colorlet{ColorLines}{black!70}
\colorlet{ColorLineMarks}{black!80}

\pgfplotsset{
    every non boxed x axis/.style={} 
}

\begin{figure}
\centering
\begin{tikzpicture}
\begin{groupplot}[
    group style={
        group name=my fancy plots,
        group size=2 by 1,
        xticklabels at=edge bottom,
        horizontal sep=12pt
    },
    height=5cm,
    ymin=1,
    ymax=185
]

\nextgroupplot[
ymin=1,
xmin=0,
xmax=220,
xtick={0,50,100,150,200},
ytick={1,50,100,150,180},
ymax=190,
height=5cm,
width=5.6cm,
clip=false,
axis y line = left,
ylabel={Persons},
xlabel={Timeline entries}
]
\addplot+ [ycomb,mark options={ColorLines},draw=ColorLineMarks] plot coordinates
	{ (0,54) (1,69) (2,180) (3,178) (4,145) (5,119) (6,116) (7,90) (8,78) (9,82) (10,49) (11,37) (12,32) (13,20) (14,19) (15,8) (16,13) (17,14) (18,5) (19,4) (20,5) (21,6) (22,4) (23,3) (24,2) (25,4) (26,3) (27,1) (28,1) (29,6) (30,3) (34,4) (35,1) (36,2) (37,1) (38,2) (39,1) (41,1) (49,1) (52,1) (61,1) (72,2) (73,1) (75,1) (78,1) (95,1) (119,1) (122,1) (125,1) (145,1) (148,1) (160,1) (210,1) };
%	\node[above] at (axis cs:160,1) {\begin{tabular}{c} Bob \\ Dole \end{tabular}};
	\node[above] at (axis cs:195,1) {\begin{tabular}{c} David \\ Beckham \end{tabular}};
\nextgroupplot[
ymin=1,
xmin=378,
xmax=405,
xtick=388,
ymax=180,
height=5cm,
width=2.6cm,
clip=false,
yticklabels={},
axis y line = right
]
\addplot+ [ycomb,mark options={ColorLines},draw=ColorLineMarks] plot coordinates
	{ (388,1) 	};
	\node[above] at (axis cs:388,1) {\begin{tabular}{c} John \\ McCain \end{tabular}};
\end{groupplot}
\end{tikzpicture}
\caption{The distribution of timeline entries per entity in the test after training the SVM classifier on the BS-BIO benchmark.}
\label{fig:benchmark_distribution}
\end{figure}

